Semantic Mapping for Orchard Environments by Merging Two-Sides Reconstructions of Tree Rows

Measuring semantic traits for phenotyping is an essential but labor-intensive activity in horticulture. Researchers often rely on manual measurements which may not be accurate for tasks such as measuring tree volume. To improve the accuracy of such measurements and to automate the process, we consider the problem of building coherent three dimensional (3D) reconstructions of orchard rows. Even though 3D reconstructions of side views can be obtained using standard mapping techniques, merging the two side-views is difficult due to the lack of overlap between the two partial reconstructions. Our first main contribution in this paper is a novel method that utilizes global features and semantic information to obtain an initial solution aligning the two sides. Our mapping approach then refines the 3D model of the entire tree row by integrating semantic information common to both sides, and extracted using our novel robust detection and fitting algorithms. Next, we present a vision system to measure semantic traits from the optimized 3D model that is built from the RGB or RGB-D data captured by only a camera. Specifically, we show how canopy volume, trunk diameter, tree height and fruit count can be automatically obtained in real orchard environments. The experiment results from multiple datasets quantitatively demonstrate the high accuracy and robustness of our method.

==> jfrGlobalAlignment.tex <==
%Consider a row of trees in an orchard. Suppose an imaging device moves along one side of the row  (which we arbitrarily call the ``front side") and captures images. Then it moves to the ``back" side and captures the second set of images.  The images can be standard RGB images or they may also include depth information. The images in each set are used to obtain two independent reconstructions represented as point clouds. 
%The main problem we address is to merge these two reconstructions by computing the scale, rotation and translation to align them. It is  formalized as follows:


At this stage, given two sets of input images $\{{\presuper{\mathcal{F}}{\mathcal{I}}}_i,{\presuper{\mathcal{B}}{\mathcal{I}}}_j\}$ from the front and back sides of a row, two corresponding reconstructions $ \{{\mathcal{F}}, {\mathcal{B}}\}$ along with extrinsic camera poses $\{{\presuper{\mathcal{F}}{\mathbf{T}}}_i,{\presuper{\mathcal{B}}{\mathbf{T}}}_j\}$  where $ i = 1, \ldots, m$ and $j = 1,\ldots, n$ of each image, the goal is to merge these two reconstructions into a single coherent model $\presuper{}{\mathcal{P}}$ with combined set of camera poses $\{\mathbf{T}\}$ by finding a transformation  $^{\mathcal{F}}_{\mathcal{B}} \mathbf{T} = s [ ^{\mathcal{F}}_{\mathcal{B}} \mathbf{R} | ^{\mathcal{F}}_{\mathcal{B}} \mathbf{t} ]$ that merges the back side reconstruction with the front (see Fig.~\ref{fig:intro_goal}).

Next, we introduce the objective function used for optimization.



\textbf{Objective Function:} The front and back side reconstructions ${\mathcal{F}}$, ${\mathcal{B}}$ generally do not share any local feature matches (point correspondences). To constrain the system, we propose to use global features based on the following observations: (1)~the occlusion boundary of an object from the front and back orthographic views are the same (see Fig.~\ref{fig:intro}(\subref{fig:Tree_Boundary})); (2)~tree trunk segments at the same height from two sides can be treated approximately as cylinders. When projected to the ground plane they share the same center of the elliptical shape. If we align the median plane of the detected trunks, the maximum depth alignment error is bounded by the trunk widths.


 
We use the following geometric concepts to formulate the optimization problem.
An orthographic front view is the parallel projection of all the points in the $XY$ plane. The occlusion boundaries of this view can be approximated by the well-known concept of alpha shapes~\cite{edelsbrunner1994three}. An alpha hull is the generalized version of the convex hull. The boundaries of an alpha hull $\alpha_{bnd}$ are point pairs that can be touched by an empty disc of radius alpha. 

In most orchard settings, there are no leaves/branches attached to the trunks near the ground plane and the number of 3D points in this region is very sparse. We can use this observation to cluster the 3D points belonging to tree trunks. Let ${\mathcal{F}}_{tr},{\mathcal{B}}_{tr}$ denote the detected trunk points close to the median trunk plane. ${\presuper{}{\mathbf{P}}}_{xy},{\presuper{}{\mathbf{P}}}_{zx}$ denotes the orthogonal projection matrix to the front and top plane. With this we can define our problem as the following minimization problem:
\begin{equation} \label{eq:base}
\scalebox{0.96}
{$
\begin{aligned}
s^*,{^{\mathcal{F}}_{\mathcal{B}}\mathbf{R}}^*, &{^{\mathcal{F}}_{\mathcal{B}}\mathbf{t}}^* = \\
\argmin_{s,^{\mathcal{F}}_{\mathcal{B}}\mathbf{R},^{\mathcal{F}}_{\mathcal{B}}\mathbf{t}} ~ &dist\left(\alpha_{bnd}\left(\mathbf{P}_{xy} \cdot {{\mathcal{F}}}\right),~ \alpha_{bnd}\left(\mathbf{P}_{xy} \cdot {^{\mathcal{F}}_{\mathcal{B}} \mathbf{T}} \cdot {{\mathcal{B}}}\right)\right) \\
+ ~ &dist\left( \mathbf{P}_{zx} \cdot {{\mathcal{F}}_{tr}}, ~ \mathbf{P}_{zx} \cdot {^{\mathcal{F}}_{\mathcal{B}} \mathbf{T}} \cdot {{\mathcal{B}}_{tr}} \right) ,
\end{aligned}
$}
\end{equation}

where $\alpha_{bnd}$ computes the alpha shape boundary points. To find similarity between two point sets $\mathcal{P},\mathcal{Q}$ in ${\rm I\!R}^D$, we use the following metric:
\begin{equation}
dist(\mathcal{P},\mathcal{Q}) = \sum_{\forall p \in \mathcal{P}} \min_{\forall q \in \mathcal{Q}} {\left(p-q\right)}^2 .
\label{eq:dist}
\end{equation}


\textbf{Technical Approach:} We can solve Eq.~\eqref{eq:base} using trusted region methods such as Levenberg-Marquardt (LM) algorithm~\cite{more1978levenberg} for which we need to find a good initial solution. Trivial initial values such as $\mathbf{I}_{3\times 3}$ and zero translation $\mathbf{0}_{3\times 1}$ do not work. 
In this paper, we develop a method to find a good initial solution. Essentially, we solve the two parts on the right-hand side of Eq.~\eqref{eq:base} sequentially along with some preliminary steps. We perform the following steps:

\begin{enumerate}
\item For both ${\mathcal{F}}, {\mathcal{B}}$, we detect the ground plane.
\item We perform a Principle Component Analysis (PCA) on both the reconstructions. Utilizing the ground plane normal, and camera poses we find the depth and up direction of the PCA components and align the point clouds roughly.
\item To get rid of the rotational component left after PCA, we perform alignment of the ground plane normals.
\item We fix the scale of the reconstructions using median scene height and fix the height of the ground plane using the median height of the ground plane inliers.
\item Now, we only have to compute the translations. We use alpha volume analysis to compute the occlusion boundary and 2D shape matching techniques~\cite{myronenko2010point} to compute the translation in the $XY$ plane.
\item Next, we align the trunk points  close to the median trunk plane
\end{enumerate}


After these steps, the point clouds are roughly aligned and the trivial initial solution $s = 1$, ${^{\mathcal{F}}_{\mathcal{B}}\mathbf{R}} = \mathbf{I}_{3\times 3}$, ${^{\mathcal{F}}_{\mathcal{B}}\mathbf{t}} = \mathbf{0}_{3\times 1}$ leads to convergence. This method does not compute the trunk overlap distance precisely. However, it provides the correspondence between the trunks from both sides.
%\todo{Wenbo: write something about your method here to continue}.
Using the Random Sample Consensus (RANSAC)~\cite{yang2010plane} scheme, the trunk and the ground area around each tree are modeled as a cylinder and a plane, respectively. This semantic information, i.e., trunks and ground areas, can be exploited into the bundle adjustment to further eliminate misalignment of two-sides reconstructions by adjusting camera poses and 3D information of semantic objects and feature points. We describe each of these steps in detail. We start with the initial step of PCA and ground plane alignment.

\subsubsection{Ground Plane Estimation and Alignment Using PCA} \label{sec:pca}
The main goal of this step is to eliminate most of the rotational difference required to align the two reconstructions. As is well known, this is normally solved by Principle Component Analysis (PCA). We assume that the length of the portion of the row covered by the input reconstruction is always longer than the height of the trees and the depth captured. Therefore, the first principle component always denotes the length of the row covered. The other two principle components though vary from reconstruction to reconstruction. Therefore, while aligning the principal components we need to be aware of which principle component denotes scene depth and which one denotes height. 

To automatically figure out the scene ``up'' and ``depth'' directions we estimate the ground plane.
We perform a simple three-point RANSAC method for plane estimation~\cite{yang2010plane}. Then, we align the corresponding principal components. If necessary, we flip the depth direction of one of the reconstructions to ensure that the frontal depth planes are opposing each other. Subsequently, we align the ground plane normals and rotate the point clouds to a canonical frame of reference $(X,Y,Z)$ where $X = [1, 0, 0]^{\top}$, $Y = [0, 1, 0]^{\top}$ (up direction) and $Z = [0, 0, 1]^{\top}$ (depth direction). Next, we fix the scale of the reconstructions using the median height of the trees (We assume that the two reconstructions are roughly the same section of the row. Otherwise, the median can be off) and fix the height of the ground plane using inliers. The reconstructions are now roughly aligned in terms of rotation and translation in $Y$ direction. Fig.~\ref{fig:inputpca} shows the result after these steps in a sample input reconstruction.
\begin{figure}[thbp]
        \centering
            \includegraphics[width =0.99\columnwidth]{figs/Wenbo/input_ICP.pdf}           
   \caption{Input and PCA Standardization. The left image shows the input to our algorithm. The right image shows the reconstructions after PCA based alignment, ground plane alignment, and scale and height adjustment. In the input, we have only six trees but in the right image, we see more than six trees. This shows that, even though most of the rotational differences are gone, the alignment is wrong in terms of translation in the $X$ direction.}
   \label{fig:inputpca}
\end{figure}

\subsubsection{Alignment of Orthographic Projection Boundaries}\label{sec: projsymmetry}

In the last section, we roughly aligned the two reconstructions in terms of rotation, scale and, translation with respect to the ground plane. Now we have to estimate translation in the canonical directions $X = [1,0,0]^{\top}$ and $Z = [0, 0, 1]^{\top}$. We start with solving for the translation in $X$ direction. In practice, reconstructions are not perfect, and the ground plane is not perfectly planar. Consequently, our estimation in the previous step contains some error in terms of rotation, scale and translation in $X \text{ and } Y$-directions. We use a method that computes this residual rotation, translation and scaling along with the translation in the $X$ direction.


As outlined in Section~\ref{sec:techoverview}, to solve this we utilize the occlusion boundary of the reconstructions from orthographic front views. We use alpha volume analysis to compute the occlusion boundaries. The alpha hull boundaries are basically a set of 2D points. Thus, essentially we are solving a 2D point set registration problem. This problem is very well studied and many solutions exist in the literature. As our alpha boundaries are noisy we use a well-known shape alignment method, Coherent Point Drift algorithm (CPD)~\cite{myronenko2010point}. Myronenko et al.~\cite{myronenko2010point} cast the point set registration problem as a probability density estimation problem. They represent one of the input point set as the centroids of a Gaussian Mixture Model (GMM) and the other input as data. For the rigid transformation case, they reparameterize the GMM centroids in terms of rotation and scale transformation. They estimate the parameters by minimizing the negative log likelihood using the Expectation-Maximization algorithm. Additionally, they add an extra component in the GMM to account for noise and outliers. At the optimum value of the parameters, two point sets are aligned. We apply the transformation computed by CPD to the entire point cloud to align them in the $XY$ directions. The top figure in Fig.~\ref{fig:occltrunk} shows the alignment of occlusion boundaries.

\begin{figure*}[thbp]
        \centering
            \includegraphics[width =\textwidth]{figs/Wenbo/merging_result1.pdf}           
   \caption{Alignment based on occlusion boundary and trunks. The left image shows how we align the occlusion boundaries of the reconstructions. The reconstructions after this step are shown in the middle image which demonstrates some alignment error in the depth direction (trunks and poles do not merge). Finally, the right image shows the merged reconstruction using trunk information which does not have any duplicate trunk/poles.}
   \label{fig:occltrunk}
\end{figure*}


\subsubsection{Alignment in Depth Direction Using Trunk Information}\label{subsubsec:trunkAlignment}

%The principle ambiguity left is the relative depth distance between the two reconstructions. In an orchard row, trees are generally planted in straight lines and tree trunks are perpendicular to the ground. Therefore, we can imagine the existences of a central trunk plane bisecting the trunks. For each individual reconstruction, this bisector plane can be approximated by the median depth-plane of the detected trunks and we can align the reconstructions roughly by aligning the points close to this median plane.
%
%\textbf{Trunk Detection:} In most orchard settings, there are no leaves/branches attached to the trunks near the ground plane. Consequently, the number of 3D points in the trunk region close to the ground is very small. We capture this region by binning the 3D points in terms of their distance from the ground plane (see Fig.~\ref{fig:trunkDetection}). The flat region in this curve shown in Fig.~\ref{fig:trunkDetection} is easily captured by utilizing the derivative. We use the region with the minimum number of points and two knee points around it to find the trunks close to the ground.
%
%\begin{figure}[thbp]
%        \centering
%            \includegraphics[width =0.80\columnwidth]{figs/Wenbo/trunk_detection.pdf}           
%   \caption{Trunk detection. Figure on the left shows the detected trunks on the simulated trees. Figure on the right shows a plot of the number of 3D points plotted against their distance from the ground plane. The flat region in this plot correspond to the 3D points belonging to the trunk regions.}
%   \label{fig:trunkDetection}
%\end{figure}
%
%We perform a simple median filtering of the trunk points ${F}_{tr},{B}_{tr}$. Then, like the previous section, we can align them using Coherent Point Drift (CPD) method~\cite{myronenko2010point}.
%
%After this step, both reconstructions are in the same frame of reference and have a very small difference in terms of rotation, translation, and scale. The trivial initial solution of $s = 1,{^{\mathcal{F}}_{\mathcal{B}} \mathbf{R}} = \mathbf{I}_{3\times 3}, {^{\mathcal{F}}_{\mathcal{B}} \mathbf{t}} = \mathbf{0}_{3\times 1}$ leads to fast convergence. The bottom figure in Fig.~\ref{fig:occltrunk} shows the merged reconstruction. As a byproduct from this process, we have established trunk to trunk correspondences between the two reconstructions. We can use this to optimize our alignment further. We discuss the details of this procedure in the next section.
%
%

